A Comprehensive Benchmark Suite for Intel SGX

Trusted execution environments (TEEs) such as \intelsgx facilitate the secure execution of an application on untrusted machines. Sadly, such environments suffer from serious limitations and performance overheads in terms of writing back data to the main memory, their interaction with the OS, and the ability to issue I/O instructions. There is thus a plethora of work that focuses on improving the performance of such environments -- this necessitates the need for a standard, widely accepted benchmark suite (something similar to SPEC and PARSEC). To the best of our knowledge, such a suite does not exist. Our suite, SGXGauge, contains a diverse set of workloads such as blockchain codes, secure machine learning algorithms, lightweight web servers, secure key-value stores, etc. We thoroughly characterizes the behavior of the benchmark suite on a native platform and on a platform that uses a library OS-based shimming layer (GrapheneSGX). We observe that the most important metrics of interest are performance counters related to paging, memory, and TLB accesses. There is an abrupt change in performance when the memory footprint starts to exceed the size of the EPC size in Intel SGX, and the library OS does not add a significant overhead (~ +- 10%).

==> evaluating_criteria.tex <==
\section{Benchmark Quality Metrics}
\label{sec:eval_criteria}

In this section, we create a novel set of criteria for evaluating the quality of 
a benchmark suite. 
The starting point is the set of properties listed qualitatively by the authors of the
PARSEC suite~\cite{parsec}.

\begin{enumerate}[1.]
\item \textbf{Diverse}: The benchmark suite should evaluate all the components of the framework that is under consideration.
\item \textbf{Phase changes:} Modern applications show different characteristics during their execution. Most synthetic or micro-benchmarks lack this feature. Hence, it is necessary to evaluate the system using real-world benchmarks.
\item \textbf{Coverage}: The benchmark suite should evaluate each component for a wide range of values. This analysis reveals how the performance changes with changing values of these components.
\end{enumerate}

We devise the following {\bf scores} to mathematically capture the aforementioned criteria.

\noindent
\textbf{Notations:}
Let us assume that our benchmark suite ($\mathcal{W}$) is a set of \textit{n} benchmarks, i.e., $\mathcal{W} = \{w_1, w_2,\dots w_n\}$. During the executing of a benchmark ($w_i \in \mathcal{W}$) we collect $m$ execution-related statistics. We store them in an $m$-dimensional vector $x_i$ for benchmark $w_i$. For a single execution of all the benchmarks in the suite, the matrix $\mathcal{X}$ contains all the individual vectors (stored as row vectors). This description is agnostic to the specific parameters captured in an execution.


\subsection{Cluster Score}
The benchmarks in a suite should be designed or chosen such as they show different properties as compared to each other in terms of execution statistics. If they are all similar to one another, running different benchmarks will reveal no additional insights. In simple terms, the benchmarks should not be {\em clustered}.

To capture the \quotes{diverse} nature of a benchmark suite, we define a score called \textit{ClusterScore}. For this, we first collect the matrix $\mathcal{X}$ to create clusters using K-means clustering~\cite{kmeans}.  To determine the quality of the clusters, we use a well-known score called the Silhouette score ~\cite{silhouette}. We want a clustering that is as {\em poor} as possible. 

\subsubsection{Silhouette Score}
Let us say we form \textit{k} clusters. For a point $p \in C_i$, i.e., point $p$ in cluster $C_i$, we first calculate an \textit{intra-cluster dissimilarity score} for the point $p$ called $\eta(p)$.

\begin{equation}
\eta(p) = \frac{1}{|C_i|-1}\sum_{\forall p'\in C_i} dis(p,p')
\end{equation}

where, $dis(p,p')$ is the Euclidean distance between $p$ and $p'$.  

After this, we calculate an \textit{inter-cluster dissimilarity score} for point $p$, i.e., $\lambda(p)$. We do this for all the clusters except for the cluster containing $p$, and then select the minimum value.

\begin{equation}
Cost(p, j) = min \frac{1}{|C_j|}\sum_{\forall p' \in C_j, C_j \ne C_i} dis(p,p')
\end{equation}
Let us define $\lambda(p)$ as the lowest cost for any $j \ne i$. 

Finally, we calculate the silhouette score for the point $p$ ($\mathcal{S}(p)$):

\begin{equation}
\mathcal{S}(p) =
\begin{cases}
 \frac{\lambda(p)-\eta(p)}{max\{\lambda(p), \eta(p)\}} & k > 1  \\
0 & \text{ if } k=1
\end{cases}
\end{equation}

The silhouette score of cluster $C_i$ is an average of the silhouette scores of all the points within that cluster.

\begin{equation}
\mathcal{S}(C_i) = \frac{1}{|C_i|}\sum_{\forall p \in C_i} \mathcal{S}(p)
\end{equation}

The silhouette score of a benchmark suite is the average of silhouette scores for all the clusters. Assuming \textit{k} clusters:
\begin{equation}
\mathcal{S}(\mathcal{W})_k = \frac{1}{k}\sum_{i=1}^{k} \mathcal{S}(C_i)
\end{equation}

%We define the metric \textit{ClusterScore} for $W$.
 To calculate the $ClusterScore$, we calculate $\mathcal{S}(\mathcal{W})_k$ for $k=2\text{ to }|\mathcal{W}|-1$, and take the average. Here, $k$ is the number of clusters.

\begin{equation}
\boxed{ClusterScore = \frac{1}{|\mathcal{W}|-2}\sum_{k=2}^{|\mathcal{W}|-1}\mathcal{S}(\mathcal{W})_k}
\end{equation}


\subsection{Trend Score}
Here, we define a metric that captures the difference between the execution trends of different workloads.
%
For a given input to a set of workloads $\mathcal{W}$ ($|\mathcal{W}|=n$), let us say $T_z = \{t_1,t_2,t_3...t_n\}$, is the set of  vectors for a particular hardware performance counter $z\in Z$ (e.g. \texttt{dTLB hits}) across all the individual workloads. Here, $Z$ is the set of all the hardware performance counters. Each  vector, $t_i$, is a time series (specific to a given workload).

To measure the distance between two time series, we use a well-known  technique called \textit{Dynamic Time Warping} or DTW~\cite{dtw1,dtw2,dtw3,dtw4}. DTW aims to minimize the distance between the two time series, which can have different lengths by non-linearly ``warping" the time-space to match them as shown in Figure ~\ref{fig:dtw}.

\begin{figure}[!ht]
\begin{subfigure}[b]{.47\linewidth}
\centering
\includegraphics[width=\linewidth]{FIGS/dtw_1.pdf}
\end{subfigure}
\hfil
\begin{subfigure}[b]{.47\linewidth}
\includegraphics[width=\linewidth]{FIGS/dtw_2.pdf}
\end{subfigure}
\caption{Figure showing Dynamic Time Warping (DTW)}
\label{fig:dtw}
\end{figure}

We calculate the pair-wise DTW distance of all the data points in $T_z$, and report the average for metric $z$ ($TScore_z$). 

\begin{align}
TScore_z = \frac{1}{|\mathcal{W}|*(|\mathcal{W}|-1)}\sum_{t_m \in T_z}\sum_{t_n \in T_z, m \ne n}DTW(t_m,t_n) 
\end{align}

We then calculate the average DTW score for all the metrics in $Z$, that is the final $TrendScore$.

\begin{equation}
\boxed{TrendScore = \frac{1}{|Z|}\sum_{\forall i \in Z }^{}TScore_i}
\end{equation}

\subsubsection{Normalization in  DTW}
Note that if a particular $t_m \in T_z$ has unusually high values (see Figure ~\ref{fig:non_cdf}), then the $TScore_z$ score will be dominated by this, and eventually the $TrendScore$~\cite{dtw4}.

To fix this, we use the CDF (cumulative distribution function)~\cite{cdf} of a particular metric instead of its absolute values. The CDF normalizes the Y-axis (see Figure ~\ref{fig:cdf}). Doing so also bounds the distance between two points to [0,100].

\begin{figure}[!ht]
\centering
\begin{subfigure}[b]{.49\linewidth}
\includegraphics[width=\linewidth]{FIGS/motivate_sgxgauge_medium_llc_misses_non_cdf_mod.pdf}
\caption{ LLC misses as a function of time}
\label{fig:non_cdf}
\end{subfigure}
\hfil
\begin{subfigure}[b]{.49\linewidth}
\includegraphics[width=\linewidth]{FIGS/motivate_sgxgauge_medium_llc_misses_cdf_mod.pdf}
\caption{ Normalizing the y-axis by considering the CDF}
\label{fig:cdf}
\end{subfigure}

\begin{subfigure}[b]{.6\linewidth}
\includegraphics[width=.9\linewidth]{FIGS/motivate_sgxgauge_medium_llc_misses_per_cdf_mod.pdf}
\caption{Normalizing the x-axis also by considering the percentage of total execution}
\label{fig:per_cdf}
\end{subfigure}

\caption{Normalizing LLC misses for workloads W1 to W5.}

\end{figure}
However, even now, the x-axis, i.e., the time axis is still not normalized because different workloads might have taken different times to execute. 
To fix this, instead of the absolute time, we use the
percentiles of the execution time to define the x-axis. The resultant normalized time series are used to compute the DTW values and ultimately the trend score ($TrendScore$).


\subsection{Coverage Score}
Here, we define a metric called \textit{CoverageScore} for a benchmark suite, that captures its spread over the parameter space (hardware counters). All the benchmarks during their execution incur different hardware events, such as TLB or LLC misses. Depending on the characteristics of the benchmarks, the value of the events can be significantly different from one another. Ideally, a benchmark suite should have a high \textit{CoverageScore}, indicating a good spread over the parameter space.


Let us assume we want to compare the coverage of two benchmarks suites $\mathcal{W}_1$ and $\mathcal{W}_2$, each containing $n$ benchmarks.

For a same (or similar) input, we execute workloads in $\mathcal{W}_1$ and $\mathcal{W}_2$ and collect the hardware counter matrices $\mathcal{X}_1$ $\mathcal{X}_2$,  respectively. All the individual parameters are normalized
and brought into the range $[0,1]$.
 
Then, we use Principal Component Analysis or PCA~\cite{pca} to reduce the dimensionality of the data, while preserving its variance. PCA will eliminate all the redundant features (events) from the data. We ensure that 98\% of the original variance is preserved.

\begin{align}
\langle \mathcal{X}^T_1, d_1 \rangle &= PCA(\mathcal{X}_1, \texttt{variance} =.98) \\
\langle \mathcal{X}^T_2, d_2 \rangle &= PCA(\mathcal{X}_2, \texttt{variance} =.98)
\end{align}

Here, $d_1$ and $d_2$ are the PCA components for the transformed  data, $\mathcal{X}_1$ and $\mathcal{X}_2$, respectively.
 We define the \textit{CoverageScore} as the variance present in the transformed data.
 

We define the \textit{CoverageScore} for $\mathcal{W}_1$ as
\begin{align}
\boxed{CoverageScore_{\mathcal{W}_1} = \frac{1}{d_1}\sum_{i=0}^{d_1-1} Variance \left ( comp_i (\mathcal{X}^T_1) \right )}
\end{align}

Here, $comp_i$ is the function that returns the contents of the $i^{th}$ PCA component. Similarly, we can calculate the CoverageScore for $\mathcal{W}_2$ also.
A high CoverageScore indicates a good coverage of the $n$-dimensional parameter space. Prior work~\cite{parsec_vs_splash} has also used a simple variance-based metric to define the coverage of PARSEC\cite{parsec} and SPLASH-2~\cite{splash_2} benchmark suites.
 


==> related_work.tex <==
%\section{Related Works}
%
%With \intelsgx gaining popularity in the past few years there are many works aiming to improve its performance and remove the limitations imposed due to security concerns. However, not much work has been done in terms of standardizing the benchmark.
%
%
%The work that most closely resembles our was done by ~\ncite{portorshim} where they modify \lmbench~\cite{lmbench} for \intelsgx. \lmbench is a suite of microbenchmark tools.
%
%SGXPerf, TEEMon, TEEPerf~\cite{sgxperf,teemon,teeperf}

